Learning to combine top-down context and feed-forward representations under ambiguity with apical and basal dendrites

One of the hallmark features of neocortical anatomy is the presence of extensive top-down projections into primary sensory areas, with many impinging on the distal apical dendrites of pyramidal neurons. While it is known that they exert a modulatory effect, altering the gain of responses, their functional role remains an active area of research. It is hypothesized that these top-down projections carry contextual information that can help animals to resolve ambiguities in sensory data. One proposed mechanism of contextual integration is a non-linear integration of distinct input streams at apical and basal dendrites of pyramidal neurons. Computationally, however, it is yet to be demonstrated how such an architecture could leverage distinct compartments for flexible contextual integration and sensory processing when both sensory and context signals can be unreliable. Here, we implement an augmented deep neural network with distinct apical and basal compartments that integrates a) contextual information from top-down projections to apical compartments, and b) sensory representations driven by bottom-up projections to basal compartments, via a biophysically inspired rule. In addition, we develop a new multi-scenario contextual integration task using a generative image modeling approach. In addition to generalizing previous contextual integration tasks, it better captures the diversity of scenarios where neither contextual nor sensory information are fully reliable. To solve this task, this model successfully learns to select among integration strategies. We find that our model outperforms those without the "apical prior" when contextual information contradicts sensory input. Altogether, this suggests that the apical prior and biophysically inspired integration rule could be key components necessary for handling the ambiguities that animals encounter in the diverse contexts of the real world.

==> legacy/discussion.tex <==
The exact mechanism by which top-down signals exert their functional role in pyramidal neurons remains unknown.  
One hypothesis is that, in the neocortex, apical dendrites of pyramidal neurons integrate top-down information from higher-order regions, which in turn modulate somatic firing rate for accurate and robust perception.
A computational framework  that respects known biophysical constraints while leveraging a task that requires integrating different types of context is ideal for testing this hypothesis.
Here, we present (1) a functional model of %(spatial) and
contextual integration at pyramidal neurons that relies on the biophysical properties of apical and basal dendrites, and (2) a novel image classification task and dataset using a conditional generative model.
Specifically for (1), we implement a Hadamard (multiplicative elementwise) integration rule based on known biophysical properties of apical dendrites which act as gain modulators of somatic activity \citep{waters_supralinear_2003, larkum_dendritic_2007}.
To solve (2), we train the top-down network (mapping of context onto apical dendrites) with the proposed loss function \ref{eq:lossfn}   by gradient descent, and assess the role of top-down signals in solving the task across 5 distinct input/context conditions.
We find that the top-down network learns to refine ambiguous representations by applying sparse gain modulation to basal signals when contextual information is both available and relevant, but also learns to ignore contradictory or irrelevant contexts.
This sparse selectivity is consistent with biased competition  in the top-down modulation of pyramidal neurons.
Our results show that it is in principle possible for local pyramidal circuits to learn a mapping of contextual representations onto their apical compartments to resolve perceptual ambiguity.
Further analysis reveals that a sparse subset of class-pair overlapping neurons are preferentially gain-modulated by top-down contextual inputs, providing a candidate mechanism for how the model solves the perceptual ambiguities.
This mixed selectivity could present distinct computational advantages across changing contexts \citep{rigotti_importance_2013}.

\subsection{Roles of top-down modulation}
Top-down feedback is a prominent feature of the neocortical architecture for which several roles have been hypothesized. 
During learning, it has been proposed to act as a credit assignment signal \citep{lee_difference_2015, guerguiev_towards_2017, meulemans_theoretical_2020, bengio_deriving_2020} and/or representing predictions \citep{rao_predictive_1999, rao_self-supervised_2022}. 
Besides its role in credit assignment, top-down feedback has also been proposed to support attentional processes \citep{lindsay_attention_2020} by dynamically highlighting the most relevant parts of an input, in both biological \citep{spratling_reconciling_2008} and artificial systems \citep{mittal_learning_2020}, and could augment sensory processing with robustness to adversarial stimuli {\citep{choksi_brain-inspired_2020} or integration of contextual or task information \citep{naumann_invariant_2022, wybo_dendritic_2022} . Given their biophysical properties, apical dendrites are particularly well poised to integrate these top-down contextual signals, and from a computational perspective, have been shown to be useful for multitask learning \citep{wybo_dendritic_2022}. Our computational framework falls into the category of updating feedforward representations. We do not exclude other hypothesized roles for top-down feedback, however their unification under one framework is outside of the scope of this work.
% Beyond adversarial noise, \citet{naumann_invariant_2022} propose that contexts can alter feedforward sensory information by rotating a high-dimensional manifold in representational space.
% In these conditions, the role of top-down signals would be to rotate these invariant representations to cancel out the effects of changing contexts.
% In the specific case of visual perception, updates to representational manifolds have been found to be provided by higher-order cortical regions \citep{morales-gregorio_neural_2023}. 

% Similar to \citep{wybo_dendritic_2022}, our model solves multiple tasks with apical dendrites via element-wise modulation of neurons' firing rates.
% Their setting differs from ours in that there is no resolution of ambiguity required, and the task is given by a task oracle, similar to our oracle case.
% - connection to uncertainty estimation 
Extending previous work on integration of topdown contextual signals via apical and basal dendrites, we focus specifically on a task in which the model must learn to differentially integrate relevant and irrelevant contextual signals at apical dendrites for accurate perception. This reflects the reality for brains, where not all contextual signals are useful or relevant to the task at hand.
% Additionally, the oracle case we present here is particularly relevant for conditions where there is no ground truth regarding stimulus identity, similar to the Necker cube classification task \citep{hardstone_long-term_2021}.
% Here we recapitulate the findings that in such conditions, perception can rely heavily on internal priors.

\subsection{Role of dendritic integration algorithms on function}
Previous models have proposed to integrate feed-forward and feedback information streams using additive \citep{mittal_learning_2020, choksi_brain-inspired_2020} ,  multiplicative \citep{naumann_invariant_2022} rules, or both \citep{wybo_dendritic_2022}.
In \citet{mittal_learning_2020}, top-down signals come from past temporal context from higher-order modules, and are integrated with the feedforward stream via additive key-value attention (\citep{vaswani_attention_2023}). These works explore similar integration rules to ours, but the mathematical forms are not equivalent.
% Besides multiplicative scaling, bias scaling, a variant of the additive rule has also been reported in ex vivo human brain tissue \citep{Larkum and Shao et al (2015)}.
Here we implement a Hadamard integration rule on the basis of a direct correspondence to biophysical principles.
While the contextual integration task can be solved using different rules \ref{tab:ablations}, under uncertainty, Hadamard integration enables the model to ignore contradictory contextual signals more efficiently compared to additive integration. Furthermore, as basal and apical signals are combined post-activation, our rule can only amplify already active neurons, unlike \cite{wybo_dendritic_2022} and \citep{naumann_invariant_2022}. From an efficiency perspective, this eliminates the need to drive other neurons to fire, and uses less of the network capacity, at the cost of expressivity. It remains to be demonstrated whether our rule enables the model to perform well for more complex tasks.

\subsection{Testable predictions}
We find that our model can learn a non-linear mapping of top-down signals onto the apical compartment, a property that was recently described in pyramidal neurons of the visual cortex \citep{fisek_cortico-cortical_2023}.
In addition to this compatibility with \emph{in vivo} conditions, we propose several key links between experimental work and our model.
Firstly, we found that under ambiguity, our model displayed a high diversity of neural responses as well as neurons that exhibit highly overlapping responses for specific class-pairs similar to \emph{in vivo} reports that subsets of pyramidal neurons display a variety of responses given a mismatch between context and sensory evidence \citep{jordan_opposing_2020, rigotti_importance_2013}.
Secondly, we find that masking apical compartments of class-pair overlapping neurons decreased task performance by a significant margin, up to nearly chance level.
This is in contrast with \emph{in vivo} experiments in non-human primates showing that inhibiting higher-order regions, and effectively shifting visual cortex representations to a strictly feed-forward regime, increased performance delays but did not prevent object recognition even for challenging images \citep{kar_fast_2021}.
Finally, our model could learn a mapping of top-down feedback to the apical compartment independent of learning contextual representations which is compatible with high-order cortical regions, including the hippocampus, learning and updating contextual representations in absence of sensory inputs and yet play a major role in memory retrieval that necessitate contextual information \citep{maren_contextual_2013}.

One key testable prediction from our model is that neurons displaying mixed-selectivity would receive the strongest top-down signals at their apical dendrites.
Testing this would require first conducting a controlled contextual integration task with an animal, and identifying a population from which a high degree of overlap is observed in neural responses for multiple categories or task variables.
We hypothesize that silencing the apical compartments of these neurons would impair the ambiguity resolution ability of the animal.

\subsection{Limitations and outlook}
While our model combines functionality with key biophysical properties of dendrites, there are some important assumptions and simplifications that need to be considered.
Firstly, our model is designed to implement some key features of cortical pyramidal neurons without focusing on a specific subpopulation that make up cortical layers, including layer 2/3 and layer 5 pyramidal neurons.
Here, we assume that contextual signals are provided by a neurons in a higher-order region, which would likely correspond to layer 5 output, and integrated in apical dendrites of putative layer 2/3 pyramidal neurons \citep{bastos_canonical_2012, schuman_neocortical_2021}.
It is noteworthy though that layer 5 neurons can also send top-down projections to the basal compartment of layer 2/3 neurons, although to a lesser extent \citep{harris_hierarchical_2019}.

Secondly, we use a deep learning framework that does not respect Dale's principle: namely, synaptic weights can be either negative and positive, giving the ability of presynaptic neurons to be both excitatory and inhibitory at the same time for distinct postsynaptic neurons.
Although our model ignores this principle, we apply normalization across inputs, which could in principle mimic a role of the inhibitory neurons if they are non-selective.
Additionally, Dale's principle could theoretically be implemented to our deep learning framework with little sacrifice in performance \citep{cornford_learning_2021}.

Our model heavily abstracts temporal dynamics that are normally observed in biological circuits.
Specifically, perception is associated with ever evolving neurophysiological responses that anchor to discrete states of sensory experience.
For example, in the presence of ambiguous stimuli, human subjects can oscillate between two interpretations, a phenomenon termed 'perceptual bistability' \citep{hardstone_long-term_2021}.
During perceptual bistability, neural activity alternates between discrete states \citep{abeles_cortical_1995, akrami_converging_2009}, following principles of continuous attractor dynamics \citep{daelli_neural_2010}.
% This continuous accumulation of evidence through time originating from multiple streams of sensory signals could dramatically contribute to improve perception.
% Here, we first present a simplified setting where context is represented by a one-hot vector which we term 'oracle case', but also propose a case where context is integrated in time, using a recurrent network.
In the future, our model could support more realistic temporal dynamics, 
%that are associated with perceptual bistability in biological systems, 
which would enable the testing of a rich array of hypotheses regarding contextual integration.

In the future, we propose that our model could be extended to hierarchies of sensory modalities interacting with each other.
Deep learning models that implement multi-modal interactions are an active area of research \citep{radford_learning_2021, alayrac_flamingo_2022, mustafa_multimodal_2022}.
In these cases, representations from each modality are mapped to a joint high dimensional space and optimized via a contrastive self-supervised training objective. 
These models do not have the explicit objective to resolve conflicting or contradictory information from other modalities.
In this context, our framework could be extended to multi-modal self-supervised learning for more robust perception in deep neural networks.
Finally, such a model could be leveraged to test specific hypotheses of contextual integration in health and disease, and in particular in cases where the physiological properties of pyramidal neurons are known to be altered \citep{kim_impaired_2014}.

==> legacy/intro.tex <==
Accurate perception relies on appropriate integration of context, as sensory signals contain incomplete or ambiguous information \citep{rao_predictive_1999, mumford_computational_1992}.
Contextual information can be derived from a number of sources, including the spatial and temporal domains \citep{eichenbaum_integration_2017}, task demands \citep{gilbert_top-down_2013}, as well as other sensory modalities.

Several key neuroanatomical and cellular features could support the computations associated with context integration.
In the mammalian brain, context has been proposed to be conveyed by top-down feedback pathways which are abundant in sensory regions of the neocortex \citep{felleman_distributed_1991, markov_anatomy_2014, harris_hierarchical_2019}.
Perturbations of top-down pathways from higher order areas have been associated with delayed object recognition \citep{kar_fast_2021} as well as disrupted stimulus response curves in lower-order regions \citep{wang_feedback_2007, nassi_corticocortical_2013}, which may reflect deficits in contextual processing.
Several feed-forward computational models of perception have implemented top-down pathways to enable object recognition of occluded images \citep{george_generative_2017, spoerer_recurrent_2017} as well as context-invariant perception \citep{naumann_invariant_2022}.

In the neocortex, pyramidal neurons are thought to integrate feedforward and top-down, feedback information at their basal and apical dendrites, respectively \citep{larkum_dendritic_2007, spruston_pyramidal_2008}.
Notably, feedback has been proposed to modulate rather than drive neuronal activities \citep{sherman_actions_1998}.
This idea is supported by the unique morphological and physiological properties of pyramidal neurons, as activity in apical dendrites in vivo is generally not sufficient to drive somatic output responses alone \citep{stuart_determinants_1998, larkum_new_1999, larkum_cellular_2013, jarvis_neuronal_2018}.
On the other hand, activation of the apical compartment has been shown to act as a gain modulator, amplifying concurrent basal activity \citep{larkum_top-down_2004}.
Combining basal and apical inputs has shown promising results for context-dependent computations (Ferrand et al., 2023), nevertheless a refinement of these principles based on real physiological properties of pyramidal neurons could be essential in scaling contextual integration.
While such physiological properties have been described extensively (see \citet{spruston_pyramidal_2008} for review), there is no consensus on the exact mechanism by which top-down signals from higher-order regions modulate somatic firing rates and update sensory representations. 
%Inevitably, experimental constraints must be enforced to test specific hypotheses about the mechanism. To shed new light on the potential mechanism, we construct a novel contextual integration task which specifically requires combining bottomup and topdown signals in order to solve it successfully. While contextual integration tasks have been proposed previously, the generation of images with controllable ambiguity is a key feature of our dataset which distinguishes it from prior work. By constructing a task from this dataset which specifically requires combining bottomup and topdown signals given biophysical constraints to solve the task, we can characterize the mechanism of topdown signals in resolving perceptual ambiguity in our model. 

% Summary
Here, we propose a functional model that learns to use context only when such information is relevant, and ignores it otherwise, ultimately learning a useful mapping of top-down contextual information onto apical compartments. 
% We apply the model in scenarios where the context is given and explore how it generalizes to situations where the context is derived by integrating spatial or temporally distributed information. 
We examine character recognition tasks in cases where the characters are ambiguous and consider two different computational settings.
First, the contextual representation is directly given to the model which learns to use this top-down input to resolve the ambiguities. 
Then, the representation of context is learned, from the 
%(spatial) or 
temporal framing of the character in words or sequences of digits. 
In both settings, we show that the model learns to use apical modulation, driven by contextual inputs, to resolve sensory ambiguities.
We find that a Hadamard (element-wise multiplicative) dendritic integration rule informed by physiological data enables strong performance in both settings of the task.

To gain insights into the learned mechanisms of top-down modulation involved in our model, we applied layer-wise relevance propagation \citep{bach_pixel-wise_2015} to identify the relative contributions of individual neurons and their apical compartments to network function.
We identified a subset of neurons that are highly relevant for class-pairs which are selectively amplified by top-down signals arriving at their apical dendrites.
We propose that, in principle, the representation of context can be learned independently from the impact that it has on ambiguity resolution.
These findings provide a candidate mechanism for how neocortical pyramidal neurons integrate top-down contextual information at their apical dendrites to support robust perception in the face of ambiguous data.
%, and a stepping stone to probing the functional role of top-down signals in more realistic and complex contextual integration tasks.

==> legacy/methods.tex <==
\subsection{Ambiguous dataset generation}
To create the dataset for our task, we first train a conditional variational autoencoder (CVAE) on standard MNIST/EMNIST  \citep{doersch_tutorial_2021, sohn_learning_2015}. 
The purpose of the CVAE in this setup is to use the learned latent space to generate images that are ambiguous between two digits.
While category-free interpolation in the latent space can be done with a vanilla VAE, the CVAE approach facilitates the generation of ambiguous images conditioned on the specified categories.
We then concatenate the input to the decoder (latent $z$) with a linear combination of one-hot vectors representing the target digits. 
We define an image to be ambiguous when it lies at the $50\% \pm 5\%$ decision boundary between two classes of a classifier trained on standard MNIST/EMNIST. We collect a set of images in triplets, where two images are unambiguous from unique classes $y_0, y_1$, and the third is ambiguous (using our criterion) between $y_0, y_1$, generated by the CVAE. This dataset format simplifies the implementation of our task setup.

\subsection{Model architecture}
The model consists of three components: the pretrained backbone, the readout for classification, and the topdown network.
We first train a variational autoencoder with a convolutional encoder and decoder to form smooth latent representations of unambiguous characters.
Once the variational autoencoder backbone is trained, its weights are frozen and a readout (MLP) is trained to classify the latent representations. 
% (spatial)  In the case of spatial context, we add an extra class that represents the absence of characters (i.e. empty location).

\subsubsection{Oracle context}
In the oracle case, top-down signals are provided in the form of a one-hot vector:
\begin{equation}
\mathbbm{1}_y(c_i):=\begin{cases}
1, & \text{if $i = y$}.\\
0, & \text{otherwise}
\end{cases}
\label{one_hot_encoding}
\end{equation}
 $\forall i \in {1\dots C}$ where C is the number of classes, $|\mathbf{c}| = C$.

%  (Spatial) \subsubsection{Spatial context}
% To extend our model to the spatial domain, we extended of the aforementioned MLP, but with variational sampling being performed using convolutional layers, so that instead integrating context in a single location, a convolutional filter covers a $n$ x $m$ grid.
% In the results presented here, we show examples for 3 x 3 grids.
% Spatial context signals are provided either as one-hot encoding in character space or as a higher-order representation (word representation).
% In the first case where context signals are provided as one-hot encoding, random characters are projected onto the spatial grid, and one randomly chosen character is made ambiguous.
% The apical compartment is then trained to rescue ambiguity at the correct location provided relevant contextual signals, and ignore unambiguous locations.
% In the second case where context signals are provided as a higher-order, word representation, the context vector consists of $n$ interleaved convolutional filters over the spatial input in a given layer, where $n$ corresponds to the length of words considered.
% This implementation ensures that the mapping of contextual signals is learned independently for each character location within a word

\subsubsection{Temporal context}
In the temporal case, context signals were provided by a Gated Recurrent Unit (GRU) network \citep{cho_learning_2014}. We trained a GRU with hidden state of size 128 to predict the modulo 10 sum of MNIST digits in a sequence of two digits'. The input to the GRU at time $t$ is not $x_t$ , but rather $\mathbf{Ub}_t$, encoded by the pretrained backbone.
After processing a sequence of digits ($x_{t-2}, x_{t-1}$), the final output state $o_t$ of the GRU was then used as a top-down context signal. 
%During training of the readout, the sequence only added up to the third digit if the third digit was ambiguous (Fig 7B, bottom row). If the third image was clean and thus identifiable via bottom-up input alone, a random sequence was provided to the GRU, which generated an incorrect expectation (Fig 7B, middle row).
    
\subsection{Training}
% Learning Rate and Optimizer
% All parameters were initialized using Kaiming-uniform distributions.
% We train each model part using Adam optimizer \citep{kingma_method_2014} using a learning rate $\eta = 1e^{-3}$ and a learning rate scheduler of step size $\sigma=10$ and factor $\gamma=0.5$.
% For the topdown network optimization, the encoder and readout are frozen.

\subsubsection{Loss function}
The topdown network $g(x, c|\Theta_a)$ is explicitly trained to minimize a loss function composed of a sum over the following 5 scenarios: ambiguous input with matching context (ambig.Match), unambiguous input with matching context (unambig.Match), unambiguous input with irrelevant context (unambig.Irrel), ambiguous input with irrelevant context (ambig.Irrel), and unambiguous input with contradictory context (unambig.Contra).
All scenarios are therefore optimized together for every gradient update step. We use mean squared error as the loss criterion between the predicted latents ( computed as in equation \ref{eq:mu_out}) and the target latents for each scenario. Each minibatch is sampled from dataset $D$, and scenarios sampled from the minibatch and set of contexts $C$.
\begin{equation}
    \mathbf{L}(\Theta_a;D) = \mathbbm{E}_{((x_0,y_0),x_{ambig},(x_1,y_1))\sim D, c_{match},c_{irrel}\sim C} [ \sum_{s=1}^5 ||\mu_s^{*}-\hat{\mu_s}||_2^2 ]
    \label{eq:lossfn}
\end{equation}
It should be noted that $x_0,x_1$ are unambiguous images sampled from $D$ . The optimum of $\Theta_a$ is given by:
\begin{equation}
    \Theta^*_a = argmin_{\Theta_a} L(\Theta_a;D)
\end{equation}
Here, $\mu_s^{*}$ is the target representation, which is for each scenario and context:

\begin{equation}
\mu_s^{*} :=\begin{cases}
\mathbf{U}\mathbf{\sigma(b_{c_{match}})}, & \text{if $s\in \{1\}$} \\
\mathbf{U}\mathbf{\sigma(b_{unambig})}, & \text{if $s\in \{2,3,5\}$} \\
\mathbf{U}\mathbf{\sigma(b_{ambig})}, & \text{if $s \in \{4\}$} \\
\end{cases}
\label{one_hot_encoding}
\end{equation}
Where $b_{c} = f(x_c|\Theta_b)$, and  $b_{unambig} = f([x_0,x_1]|\Theta_b)$. Predicted latents are given by:

\begin{equation}
\hat{\mu}_s :=\begin{cases}
\mathbf{U}\mathbf{\sigma(b_{ambig})\odot(1+\sigma(a_{b_{ambig},c_{match}}))}, & \text{if $s\in \{1\}$} \\
\mathbf{U}\mathbf{\sigma(b_{unambig})\odot(1+\sigma(a_{b_{unambig},c_{match}}})), & \text{if $s\in \{2\}$} \\
\mathbf{U}\mathbf{\sigma(b_{unambig})\odot(1+\sigma(a_{b_{unambig},c_{irrel}}})), & \text{if $s\in \{3\}$} \\
\mathbf{U}\mathbf{\sigma(b_{ambig})\odot(1+\sigma(a_{b_{ambig},c_{irrel}}))}, & \text{if $s \in \{4\}$} \\
\mathbf{U}\mathbf{\sigma(b_{unambig})\odot(1+\sigma(a_{b_{unambig},c_{contra}}})), & \text{if $s\in \{5\}$} \\
\end{cases}
\label{one_hot_encoding}
\end{equation}
Where $\mathbf{a_{b,c}} = {g(\mathbf{Ub,c}|\Theta_a)}$ (See pseudocode \ref{alg1})

\begin{algorithm}
\caption{Training of the top-down model with oracle context}\label{alg1}
\begin{algorithmic}[1]
\Require Dataset $D$, learning rate $\lambda$, dimension of basal activation $d_b$, number of classes $C$, top-down input $\mathbb{R}^{d_b+C}$, output:  $\mathbb{R}^{d_b}$, bottom-up network (frozen) $f_{\Theta_b}$, latent projection (frozen) $\mathbf{U}$, top-down network $g(\dot|{\Theta_a})$, batch size B\\
\State $\mathbf{\Theta}_{a} \gets \texttt{init\_kaiming()}$
    \For {$\texttt{triplet minibatch} (\mathbf{x_0},\mathbf{y_0}), \mathbf{x_{ambig}}, (\mathbf{x_1},\mathbf{y_1}) \texttt{ sampled from } D$}
        \State $y \gets \{\mathbf{y_0}, \mathbf{y_1}\}$
        \State $x \gets \{\mathbf{x_0, x_1} \}$
        \State $\texttt{\# Concatenate all scenarios into single batch}$
        \State $\mathbf{c_{match}} \gets random\_choice(y,size=B)$  \texttt{ \# Sample context uniformly from y over minibatch}
        \State $\mathbf{c_{irrel}} \gets random\_choice(range(C) \not\in y,size=B)          \texttt{ \# Sample context uniformly (excluding S)}$
        \State $\mathbf{c_{contra}} \gets \mathbf{y_1}$
        \State \text{\# combine all vectors into one for efficiency}
        \State $c \gets cat(c_{match},c_{match},c_{irrel},c_{irrel},c_{contra})$
        \State
        $\mu^* \gets cat(\mu_{c_{match}}, \mu_{y}, \mu_{y}, \mu_{ambig}, \mu_{y_0})$
        \State
        $x \gets (x_{ambig}, x, x, x_{ambig},x_{0})$
        \State
        $b \gets f(x;\Theta_b)$
        \State 
        $a \gets g(\mathbf{U}b\oplus c ; \Theta_a) $
        \State
        $\mathbf{\hat{h}} \gets \textbf{relu}(b) \odot (1 + \textbf{relu}(a))$
        \State
        $\mathbf{\hat{\mu}} \gets \mathbf{U\hat{h}}$
        \State
        $Loss \gets \textbf{mse}(\mathbf{\hat{\mu}}, \mu^*)$
        \State $\texttt{\# autograd optimizer step}$
        \State $\Theta_a \gets \Theta_a + \lambda \nabla_{\Theta_a} Loss$
      \EndFor
\end{algorithmic}
\end{algorithm}


\subsubsection{Layer-wise Relevance Propagation Analysis}
We applied layer-wise relevance propagation (LRP) to identify specific neurons whose activity, as described by $\mathbf{h}$ in our model, contributed most to the category readouts. For this analysis, we trained a readout to classify the standard categories (ie. digits 0-9) as well as all possible ambiguous pairs (ie. 3/5, 5/8, 1/7, etc.), which for MNIST gives a total number of categories $C=55$. To identify the subset of neurons that are most relevant for a given class $i$, we sorted neurons by highest to lowest average relevance per class.
We then computed the normalized cumulative sum of relevance of neurons, and define $S_i$ as the minimum set of neurons required to obtained 95\% of the total LRP for each class $i$ where $i \in {0,1, \cdots, C}$  (fig.~\ref{fig:results_LRP_analysis}\textbf{d}).
We computed the separability between sets $S_{i}$, $S_{j}$ as $1-|S_{i} \cap S_{j}| / |S_{i} \cup S_{j}|$ (Fig.~\ref{fig:results_LRP_analysis}\textbf{e}). 

\subsection{Statistical analysis}
Parametric tests where used when data distribution was normal and variance homogeneous, otherwise non-parametric tests were used and reported when appropriate.
\textbf{Meaning of abbreviated statistical terms}. 1-ANOVA: one-way ANOVA; 2-ANOVA, two-way ANOVA; RM-ANOVA, repeated-measure ANOVA.
Error bars and bands represent standard error of the mean, unless stated otherwise.
*, p $<$ 0.05; **, p $<$ 0.01; ***, p $<$ 0.001; ****, p $<$ 0.0001; n.s., not significant.

\subsection{Code availability}
All experiments were carried out using PyTorch.
% (Paszke et al., 2019).
We use the MNIST and EMNIST datasets,
% (Deng et al., 2012). 
where number of output classes are $C = 10$ for MNIST, and $C = 26$ for EMNIST.
The code for models and data analysis is publicly available under: 
https://github.com/ABL-Lab/expectation-clamp
The code used to generate the ambiguous datasets as well as links to pre-generated datasets are available under:
https://github.com/ABL-Lab/ambiguous-dataset

==> legacy/results.tex <==
\subsection{Functional model of context integration in apical dendrites}
To model how apical dendrites integrate context to refine perceptual representations, we developed a task where correct classification of ambiguous characters requires appropriate integration of contextual cues (Fig.~\ref{fig:fig1}\textbf{a}).
In this task, we trained a generative model to construct a dataset of ambiguous handwritten digits and letters based on MNIST and EMNIST, respectively. 
This generative model synthesizes images that are ambiguous between pairs of classes (see Methods).
The resulting ambiguity was empirically quantified with a linear classifier trained on unambiguous images (fig.~\ref{fig:fig1}\textbf{b}).
Inspired by anatomical features of pyramidal neurons, we next developed a model that implements distinct dendritic compartments, a basal compartment for integrating sensory information and an apical compartment for integrating contextual information (Fig.~\ref{fig:fig1}\textbf{c}).
In the model, a population of $n$ pyramidal neurons has two sources of inputs, represented as vectors: a set of basal inputs, $\mathbf{b} = [b_1, \hdots, b_n]$, representing the sensory stream, and a set of apical inputs, $\mathbf{a} = [a_1, \hdots, a_n]$, representing the top-down stream.
Input images, $\mathbf{x}$, are encoded by a pretrained network $f$, with parameters $\Theta_b$.
$f$ is a convolutional neural network reflecting initial stages of sensory processing (see Methods for more details on how the encoder is pretrained).
The output of $f(x)$ is the basal vector $\mathbf{b}$.
% The basal input vector is then calculated using these encoded sensory inputs and a synaptic weight matrix, $$, which represents the basal synaptic weights, $W_{ij}$, where $j$ is an index over elements in the output of the encoder.
% The resulting equation is: 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{equation}
% \mathbf{b} = \mathbf{W} f(\mathbf{x}).
% \label{eq:basal_compartment}
% \end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The firing rate of pyramidal neurons, $\mathbf{h} = [h_1, \hdots, h_n]$, is then determined by a thresholded element-wise (neuron-wise) combination of the basal and apical input vectors:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\mathbf{h} = \sigma(\mathbf{b}) \odot (\sigma(\mathbf{a})+1),
\label{eq:soma_output}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

where $\odot$ is an element-wise multiplication and $\sigma$ is the rectified linear unit (ReLU) activation function.
We refer to this integration rule as 'Hadamard'.
As can be seen from equation \ref{eq:soma_output}, the impact of the apical input vector, $\mathbf{a}$, on the firing rate, $\mathbf{h}$, is determined by $\sigma(\mathbf{a})+1$, which has elements that are by design always greater than or equal to one. 
As such, the apical activity serves as a thresholded neuron-wise gain modulator of the basal activity. 
This modulated basal activity is ultimately the firing rate of the modelled neurons, in-line with previous experimental findings \citep{waters_supralinear_2003}. 
Under these constraints, apical inputs affect neuronal activity only under the condition that they exceed their activation threshold (when $a > 0$), similar to the requirement for regenerative calcium spikes for apical inputs to influence somatic spiking in real pyramidal neurons \citep{larkum_new_1999}.
The output of the model is read-out from a feedforward linear transformation of the pyramidal neurons firing rates:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:mu_out}
\mathbf{\mu} = \mathbf{U} \mathbf{h},
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

where $$\mathbf{U}$$ is a pretrained linear transformation and $\mu$ represents a higher-order neuronal population.
To obtain the apical inputs $\mathbf{a}$, the context, $\mathbf{c}$, (which is either derived from 
%(spatial) or 
temporal context, or given directly, see below) is merged with the output and mapped onto the apical compartment using a multilayer perceptron (MLP), $g(\cdot)$, as follows:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\mathbf{a} = g(\mathbf{c} \oplus \mathbf{U\sigma{(b)}}),
\label{apical_compartment}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\oplus$ is the concatenation operation, $\sigma$ is the ReLU activation, and $g$ is a 2-layer MLP (1 hidden layer) with learnable parameters denoted by $\Theta_a$.
The model must use the combination of context and input to determine the representation of both ambiguous and unambiguous characters. 
For ambiguous characters, which are a mixture of two categories, the readout of the representations of the model will yield two plausible interpretations (one corresponding to the target category, and one corresponding to the contradictory category).
The contradictory category refers to the class that induces the most confounding readout classification.
Categories other than the target or contradictory we refer to as irrelevant categories. 
To test whether the model can learn useful apical modulations, we trained the synaptic weights $\Theta_a$ with the objective $L$ of modulating basal representations to match the target latent representations under various scenarios of input and context by gradient descent; Fig.~\ref{fig:fig1}\textbf{e}; pseudocode \ref{alg1}, and \ref{eq:lossfn})
This setup ensures that the top-down model is trained on both unambiguous and ambiguous samples, and that the model must learn to provide the appropriate modulatory signal only when it is relevant, ensuring that our model could learn to ignore contextual information when appropriate.
This implementation reflects the fact that, in the mammalian brain, top-down modulation is available from multiple sources and present regardless of whether the sensory inputs are ambiguous or not, and whether the contextual sources are helpful for resolving ambiguity or not. 

This suggests an approach where the problem of contextual integration is broken into two parts:
(1) how apical dendrites locally learn to use contextual representations $c$ to solve the task and (2) how those contextual representations $c$ can be learned from the 
%(spatial)and 
temporal frame.

For the first part, our initial experiments assume that context, $c$, is given in the form of a one-hot vector, a scenario we refer to as the 'oracle context' (see Methods).
Subsequent experiments for the second part address the problem of learning a representation of context, $c$, taking inspiration from the neocortex, where context is, in part, represented by higher-order regions with broader windows of 
%(spatial) and 
temporal integration \citep{eichenbaum_integration_2017} (Fig.~\ref{fig:fig1}\textbf{c}; see Methods).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % [scale=1]->[width=/linewidth]
\begin{figure}[htp]
\includegraphics[width=\linewidth]{figure1.pdf}
\caption{\textbf{Functional model of context integration in apical dendrites}. 
\textbf{a}, in our experimental paradigm, ambiguous characters (in yellow, top panels) are resolved by combining context signals (bottom panels).
\textbf{b}, examples of unambiguous pairs and resulting ambiguous characters generated using EMNIST (left) and MNIST (right).
\textbf{c}, model of pyramidal neurons with distinct dendritic compartments trained to solve a task of perceptual ambiguity. Before top-down modulation, two predictions have equal probability. After top-down modulation, context contributes to favoring one unambiguous representation.
\textbf{d}, model implementation of dendritic integration using a hierarchical convolutional neural network.
\textbf{e}, distinct combinations of input and context used to train the top-down network $g$.
\textbf{f}, possible combinations of input and context used during training and analysis.
}
\label{fig:fig1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resolving ambiguity in the oracle context}
To first test if our model can categorize digits under contextual input represented as a one-hot vector (oracle context), we trained $g$ on the ambiguous MNIST/EMNIST task with a loss including all 5 scenarios of stimulus and context (see Methods). 
We assessed performance of the model in each scenario as the held-out test set accuracy on the pretrained category readout.
and found model performance was significantly modulated by top-down signals (one-way ANOVA; $F_{4}$ = 10076.598; p $<$ 0.0001; n = 313 independent samples).
Test set accuracy on ambiguous digits was $44.619 \pm 8.073\%$ without top-down modulation, and became significantly higher with top-down modulation ($99.491 \pm 1.306\%$; Tukey's test; p $<$ 0.0001) if context was matching, but did not improve performance if context was irrelevant ($43.920 \pm 8.160$; Tukey's test; p = 0.4651; n = 313 independent replicates; Fig.~\ref{fig:fig2}\textbf{a};  Table \ref{tab:results}). 

Importantly, the model did not learn to rely solely on top-down context, since performance for unambiguous input and contradictory context remained high (Fig.~\ref{fig:fig2}\textbf{a}; \ref{tab:results}).
To visualize the ability of our model to disambiguate on a population level, we projected the model output $\mathbf{\mu}$ onto a two-dimensional manifold using t-SNE (\cite{maaten_visualizing_2008}; Fig.~\ref{fig:fig2}\textbf{b}).
Ambiguous images that were initially associated with overlapping clusters were effectively disentangled after integrating matching contextual inputs (paired t-test, t$_{99}$ = 6.0293, p $<$ 0.0001 for silhouette scores between ambiguous images before and after integrating top-down inputs; Fig.~\ref{fig:fig2}\textbf{c}).
These results show that our model learned to use contextual inputs provided to apical dendrites in the form of a one-hot encoding to modulate basal activity and resolve ambiguity in sensory inputs.

\begin{figure}[htp]
\includegraphics[width=\linewidth]{figure2.pdf}
\caption{\textbf{Ambiguity can be resolved only when integrating top-down signals}.
\textbf{a}, readout test set accuracy before and after combining top-down signals over training epochs for all input-context combinations. Dashed line corresponds to chance level.
\textbf{b}, low dimensional projection (t-SNE) of $h$ for unambiguous inputs (top), ambiguous inputs before (bottom left), and after (bottom right) top-down modulation.
\textbf{c}, silhouette scores for $h$, for each class pair and for unambiguous inputs (left), ambiguous inputs before (center), and after (right) top-down modulation.
\textbf{d}, cosine distance between $h$ in unambiguous conditions and basal, apical compartments and firing rate in each scenario.
}
\label{fig:fig2}
\end{figure}

Next, we evaluated the importance of the bio-inspired integration rule (Hadamard) and an arithmetic sum of basal and apical activities (\ref{fig:results_integration}\textbf{a}).
When inputs are ambiguous and context is useful, we find that the Hadamard integration rule outperforms arithmetic summation specifically when said context is associated with high levels of certainty (represented by a context vector with values $>$ 0.8 for the target class; RM-ANOVA, F$_{8}$ = 53.0945, p $=$ 0.0001 for the interaction between integration rule and contextual certainty; \ref{fig:results_integration}\textbf{b}).
Interestingly, when inputs were unambiguous and context contradictory, the Hadamard integration rule only outperformed arithmetic summation for lower values of contextual certainty (RM-ANOVA, F$_{8}$ = 19.3529, p $=$ 0.0023 for the interaction between integration rule and contextual certainty; \ref{fig:results_integration}\textbf{c}).

\begin{figure}[htp]
\includegraphics[width=\linewidth]{figure_integration.pdf}
\caption{\textbf{Role of integration rules on ambiguity resolution}. \textbf{a}, comparison between Hadamard and arithmetic sum integration rules. \textbf{b}, test set accuracy relative to contextual certainty using either integration rule in conditions where inputs are ambiguous and context is useful.
\textbf{c}, same but in conditions where inputs are unambiguous and context contradicts the true label.} 
\label{fig:results_integration}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Single neuron mechanisms of top-down modulation}
We next sought to understand the computational role played by top-down modulation of pyramidal apical dendrites in solving this contextual integration task.
To this end, we developed a method to identify neurons relevant for solving the task.
We then analysed their activations across the various contextualized input conditions to reveal the differential role played by their apical compartments.
First, to define the sub-populations of pyramidal neurons performing specific computations, we employed layer-wise relevance propagation (LRP; \citep{bach_pixel-wise_2015}; supplementary Fig.~\ref{fig:results_LRP_analysis}\textbf{a}), a method typically used to explain which regions of an input contribute most to model output.
Specifically, each neuron receives a score for its contribution to the model output for each image (Supplementary Fig.~\ref{fig:results_LRP_analysis}\textbf{b}).
We then defined the subset of neurons most relevant for identifying a given class, $S_C$, as the minimum set of neurons required to account for 95\% of total neuronal relevance when processing images from that class (Fig. ~\ref{fig:results_LRP_analysis}\textbf{c,d}, see Methods).
Sets of relevant neurons defined in this way exhibit low overlap between classes (Supplementary Fig.~\ref{fig:results_LRP_analysis}\textbf{b-d}, see Methods).
We observed similar representational separability between classes for other scenario and given appropriate top-down inputs (Supplementary Fig.~\ref{fig:results_LRP_analysis}\textbf{e}).
Additionally, these sets of relevant neurons are typically sparse and represent $\sim$15\% of the total neuronal population(Supplementary Fig.~\ref{fig:results_LRP_analysis}\textbf{b,c}).

It is noteworthy that the model is not explicitly provided with the ambiguous nature of input images, and therefore learns to extract this information to solve the task.
In addition, the model learns to ignore top-down signals when the image is unambiguous and context is contradictory.
Given that the apical compartment must combine contextual information and the contextually naive output differentially depending on the ambiguity of the input, we hypothesized that solving the task effectively required the modulation of a subset of neurons encoding overlapping or entangled features for  each class pair.
To assess this possibility, we registered the amplitude of apical signals arriving at LRP subsets pertaining to class-specific neurons and class-pair overlapping neurons in each scenario (Fig.~\ref{fig:results_neuron_mechanisms}\textbf{a-f}).
When comparing all input/context scenarios, we found that apical signals were highest when input images were ambiguous and context informative (1-ANOVA, F$_{416}$=237.024, p $<$ 0.0001, for the main effect of input/context scenario; Fig.~\ref{fig:results_neuron_mechanisms}\textbf{b}).
Across all scenarios, neurons most relevant for class-pairs were associated with the highest amplitude in the apical compartment (1-ANOVA, F$_{417}$=17.9445, p $<$ 0.0001, for the main effect of neuron class; Fig.~\ref{fig:results_neuron_mechanisms}\textbf{b}).
We hypothesized that class-pair overlapping neurons are also most modulated by top-down context, and that modulating these neurons is necessary to solve the perceptual ambiguity classification task (Fig.~\ref{fig:results_neuron_mechanisms}\textbf{c}).

To evaluate this hypothesis, we applied a mask on selected neurons at inference time and assessed the model's performance.
Specifically, we assess readout test set accuracy when inputs are ambiguous and context is helpful, and compare cases where class-pair overlapping neurons (as identified with LRP) are specifically masked (by setting their value to 0) to cases where other randomly selected neurons are masked.
We also evaluate the effect of mask size and found that masking class-pair overlapping neurons specifically lead to significantly more rapid degradation of accuracy with increasing mask size compared to other neurons (Fig.~\ref{fig:results_neuron_mechanisms}\textbf{d}).
This highlights the key role of these neurons' apical compartments in integrating relevant contextual signals.

\begin{figure}[htp]
\includegraphics[width=\linewidth]{figure_neuron_mechanisms.pdf}
\caption{\textbf{Class-pair overlapping neurons receive the strongest top-down signals}. 
\textbf{a}, using layer-wise relevance propagation, we identify neurons most relevant for either of two classes (red and blue), or overlap of both classes (magenta).
\textbf{b}, amplitude of the apical compartment (normalized over all neurons) for each input/context condition. Three distinct classes of neurons are compared: neurons most relevant for unambiguous class A (blue), B (red), or neurons most relevant for both A and B classes (magenta).
\textbf{c}, we hypothesize that class-pair overlapping neurons receive the highest amplitude of top-down signals when processing ambiguous images, especially given matching context.
} 
\label{fig:results_neuron_mechanisms}
\end{figure}

% \subsection{Topdown network learns distinct context embeddings (TODO)}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{context_embedding_similarity2.png}
%     \caption{Caption}
%     \label{fig:embeddings}
% \end{figure}
% Due to oracle context $c$ being onehot encoded, we can rewrite the hidden topdown activation (before output $\mathbf{a}$) as $h^{apical} = h'_{apical} + e_i, \text{ } h^{apical},e_i \in \mathbbm{R}^d$ where i is the nonzero index, $e_i = W^1_{context}c$ is the embedding, '+' is elementwise addition, and $h'_{apical} = W^1_{apical} \mu$. This is simply separating $W^1$ into its components $W^1_{apical}, W^1_{context}$. in \ref{fig:embeddings}, we observe the cosine similarity across contexts in the initial, random embeddings and the resulting learned embeddings.

% \subsection{Dimensionality reduction reveals divergence of relevant and irrelevant activation distributions (TODO)}

% \subsection{Deriving context from spatial information} (spatial)
% Given that our model could solve a perceptual ambiguity task in conditions where context is given (i.e. as a one-hot encoding), we next evaluated whether contextual representations could be learned and leveraged by our top-down model.
% We first extend our model to cases where context is derived from spatial contextual information.
% Specifically, we devised a task where individual characters are displayed in the spatial domain and can be combined to form words or numbers.
% For each image, one character is ambiguous and contextual cues are provided by the higher-order representations (Fig.~\ref{fig:results_spatial}\textbf{a}, center).
% Specifically, these higher-order contextual representations can be directly given (oracle context) or learned (word context) to ultimately rescue ambiguous representations at the hierarchical level of individual characters (Fig.~\ref{fig:results_spatial}\textbf{b}).
% For this latter case, we implemented interleaved convolutions to propagate distinct representations at the character level, from a single higher-order word representation (see Methods).
% For the oracle context condition, we find that we can rescue ambiguous representations to 95.04\% $\pm$ 0.58 accuracy after integrating top-down context (paired t-test, t$_{99}$ = 36.9303, p $<$ 0.0001; Fig.~\ref{fig:results_spatial}\textbf{c}).
% Since our model learns representations using an autoencoder objective, we could decode spatial representations before and after contextual integration and found that while ambiguous characters were effectively updated into plausible unambiguous representations, unambiguous characters remained unaffected (Fig.~\ref{fig:results_spatial}\textbf{d}).
% In conditions where the context is provided by a higher-order representation (word context), we find that top-down context can effectively rescue ambiguous characters with 85.66 $\pm$ 1.16 accuracy by leveraging word representations (paired t-test, t$_{99}$ = 26.5931, p $<$ 0.0001; Fig.~\ref{fig:results_spatial}\textbf{e}).

% \begin{figure}[htp]
% \includegraphics[width=\linewidth]{figure_spatial_expectation.pdf}
% \caption{\textbf{Deriving context from spatial information}.
% \textbf{a}, we extended our classification task to the spatial domain where two distinct hierarchical levels are considered: character and word levels. As one of the characters is ambiguous, the model learns to update representations in space using higher-order word context.
% \textbf{b}, a 1x3 convolution was trained to read-out latent activations associated with words at each grid location. We then used 1x1 or 1x3 convolutions to propagate top-down context from either characters or words, respectively.
% \textbf{c}, pretrained readout classification accuracy on ambiguous characters, before and after integrating top-down oracle context.
% \textbf{d}, decoder reconstructions of unambiguous target (left), ambiguous inputs (center), and updated representation after combining top-down context (right). Red arrow indicates location of ambiguous character).
% \textbf{e}, pretrained readout classification accuracy on ambiguous characters, before and after integrating top-down word context. Each line represents accuracies on distinct images.
% }
% \label{fig:results_spatial}
% \end{figure}

\subsection{Deriving context from temporal information}
Contextual priors can also be extracted from the temporal domain, specifically by leveraging past information to decode incoming ambiguous sensory inputs.
To extend our model to cases where contextual signals are derived from the temporal domain, we trained a Gated Recurrent Unit (GRU) network to predict the arithmetic sum of two unambiguous digits as encoded by our pretrained feedforward weights $\mathbf{\Theta_b}$.
The final output state of the GRU was then given as a contextual signal for our model.  (fig.~\ref{fig:results_temporal}\textbf{a}; see Methods).
We find that in cases where the input is ambiguous and the temporal sequence sums to a plausible interpretation of the ambiguous image, the model updates perceptual representations using contextual signals to successfully resolve ambiguities (fig.~\ref{fig:results_temporal}\textbf{b}, top).
Importantly, context is effectively ignored in cases where input is unambiguous and contextual signals irrelevant (fig.~\ref{fig:results_temporal}\textbf{b}, bottom).
Using low-dimensional projections of latent representations, we find that top-down context derived from the temporal domain effectively disentangled overlapping representations when inputs are ambiguous, similarly to the oracle case. (fig.~\ref{fig:results_temporal}\textbf{c})

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
  \begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lllllll@{}}
\toprule
Task & context & ambig.Match & unambig.Match & unambig.Irrel & ambig.Irrel & unambig.Contra  \\ \midrule
 MNIST & oracle & 0.996 $\pm$ 0.000 & 0.983 $\pm$ 0.001 & 0.979 $\pm$ 0.002 & 0.461 $\pm$ 0.003 & 0.964 $\pm$ 0.001 \\
 MNIST  & temporal & 0.963 $\pm$ 0.001 & 0.999 $\pm$ 0.000  & 0.991 $\pm$  0.001 & 0.487 $\pm$ 0.005 & 0.990 $\pm$  0.001 \\
EMNIST & oracle & 0.993 $\pm$ 0.001 & 0.969 $\pm$ 0.003 & 0.936 $\pm$ 0.003 & 0.469 $\pm$ 0.004 & 0.903 $\pm$ 0.002 \\                
\end{tabular}
\end{adjustbox}
\caption{Readout test set accuracy on MNIST and EMNIST with different context representations. Results are expressed for each scenario as mean \% $\pm$ standard deviation.}
\label{tab:results}
\end{table}

\begin{figure}[htp]
\includegraphics[width=\linewidth]{figure_temporal_expectation.pdf}
\caption{\textbf{Deriving context from temporal information}. \textbf{a}, rationale for training a model that leverages context derived from temporal sequences through a recurrent network (GRU). 
\textbf{b}, example sequence used to generate context signals (as the arithmetic sum of two digits, left and center columns) to resolve ambiguity of an input image (right column). 
\textbf{c}, t-SNE projection of latent representation associated with ambiguous inputs before (left) and after (right) combining top-down signals.}
\label{fig:results_temporal}
\end{figure}

% \begin{figure}
%     \centering\includegraphics{progressive_masking_placeholder.png}
%     \caption{(TODO: replace placeholder with new data) Causal effect of progressively masking top relevant neurons' apical compartments for different conditions on accuracy in  ambig.ExpM (S1) scenario.}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{mock_orthogonal_apical.png}
%     \caption{(TODO: replace mock figure) Illustration of the topdown decision to modulate neuronal firing rates based on detecting matching (on-target, relevant) or non-matching (off-target, irrelevant) context. Throughout the course of training, the topdown network learns intermediate apical representations (1) which are orthogonal to the outer apical weight matrix (2) when context is irrelevant, such that the final apical output computed by the dot product of (1) and (2) produces near 0 magnitude. When context is relevant, the two are not orthogonal, as shown in the figure, resulting in a final output that is non-zero.}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering\includegraphics{mock_causal_mask_manifold_effect.png}
%     \caption{(TODO: Replace mock figure) The causal role of masking out top relevant neurons for different conditions on the displacement of the latent representation in the manifold from the target.}
%     \label{fig:enter-label}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}llllllll@{}}
\toprule
ambig.Match & unambig.Match & unambig.Irrel & ambig.Irrel & unambig.Contra & modulation & context\_only &  \\ \midrule 
0.989 $\pm$ 0.002 & 0.959 $\pm$ 0.003 & 0.931 $\pm$ 0.004 & 0.469 $\pm$ 0.003 & 0.841 $\pm$ 0.004 & concat   & 0 \\
0.794 $\pm$ 0.005 & 0.967 $\pm$ 0.003 & 0.938 $\pm$ 0.003 & 0.473 $\pm$ 0.004 & 0.903 $\pm$ 0.014 & concat   & 1 \\
0.993 $\pm$ 0.001 & 0.969 $\pm$ 0.003 & 0.936 $\pm$ 0.003 & 0.469 $\pm$ 0.004 & 0.903 $\pm$ 0.001 & hadamard & 0 \\
0.913 $\pm$ 0.008 & 0.929 $\pm$ 0.004 & 0.901 $\pm$ 0.006 & 0.468 $\pm$ 0.005 & 0.738 $\pm$ 0.008 & hadamard & 1 \\
0.994 $\pm$ 0.001 & 0.974 $\pm$ 0.001 & 0.944 $\pm$ 0.001 & 0.466 $\pm$ 0.007 & 0.920 $\pm$ 0.001 & sum      & 0 \\
0.792 $\pm$ 0.011 & 0.967 $\pm$ 0.005 & 0.937 $\pm$ 0.003 & 0.462 $\pm$ 0.013 & 0.904 $\pm$ 0.008 & sum      & 1\\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Ablation experiments on EMNIST for the integration rule. Context only $= 0$ when the topdown network has access to feedforward latent $\mathbf{Ub}$ and $c$ (standard case), and context only $=1$ when only $c$ is provided as input. Three modulation (integration) rules are tested: hadamard (ours), sum, and concat (see \ref{fig:results_integration}. Concat refers to a concatenation of 'topdown' weights on the basal weight matrix, akin to adding dendritic branches on the basal compartment.}
\label{tab:ablations}
\end{table}






